Recurrent U-Net for Resource-Constrained Segmentation

State-of-the-art segmentation methods rely on very deep networks that are not always easy to train without very large training datasets and tend to be relatively slow to run on standard GPUs. In this paper, we introduce a novel recurrent U-Net architecture that preserves the compactness of the original U-Net, while substantially increasing its performance to the point where it outperforms the state of the art on several benchmarks. We will demonstrate its effectiveness for several tasks, including hand segmentation, retina vessel segmentation, and road segmentation. We also introduce a large-scale dataset for hand segmentation.

==> dataset.tex <==
% !TEX root = top.tex
% !TEX spellcheck = en-US


We report the performance of our approach on standard hand-segmentation benchmarks, such as GTEA~\cite{Fathi11}, EYTH~\cite{Urooj18}, EgoHand~\cite{Bambach15}, and HOF~\cite{Urooj18}. These, however, are relatively small, with at most 4,800 images in total, as can be seen in Table~\ref{tab:dsComp}. To evaluate our approach on a larger  dataset, we therefore acquired our own. Because this work was initially motivated by an augmented virtuality project whose goal is to allow someone to type on a keyboard while wearing a head-mounted display, we asked 50 people to type on 9 keyboards while wearing an HTC Vive~\cite{HTCvive}. To make this easier, we created a mixed-reality application to allow the users to see both the camera view and a virtual browser showing the text being typed.  To ensure diversity, we varied the keyboard types, lighting conditions, desk colors, and objects lying on them, as can be seen in Fig.~\ref{fig:annotEx}.  We provide additional details in Table~\ref{tab:kbh}. 


We then recorded 161 hand sequences with the device's camera.   We split them as 20/ 20/ 60\% for train/ validation/ test to set up a challenging scenario in which the training data is not overabundant and to test the scalability and generalizability of the trained models. We guaranteed that the same person never appears in more than one of these splits by using people's IDs during partitioning. In other words, our splits resulted in three groups of 30, 30, and 101 separate videos, respectively. 
We annotated about the same number of frames in each one of the videos, resulting in a total of 12,536 annotated frames. 
%\MS{Removed the description of the annotation tool.}
%To this end, we developed a tool based on OpenCV's implementation of Grabcut~\cite{Rother04}. In practice, the annotator provides a few hard labels, in the form of short segments drawn with the mouse, and an initial segmentation is obtained using the graph-cut algorithm. The annotator can then iteratively refine this segmentation by incorporating new hard labels. Fig.~\ref{fig:annotEx} depicts the resulting ground-truth segmentations in a few frames. 

